Scilla: a Smart Contract Intermediate-Level LAnguage

This paper outlines key design principles of Scilla---an intermediate-level language for verified smart contracts. Scilla provides a clean separation between the communication aspect of smart contracts on a blockchain, allowing for the rich interaction patterns, and a programming component, which enjoys principled semantics and is amenable to formal verification. Scilla is not meant to be a high-level programming language, and we are going to use it as a translation target for high-level languages, such as Solidity, for performing program analysis and verification, before further compilation to an executable bytecode. We describe the automata-based model of Scilla, present its programming component and show how contract definitions in terms of automata streamline the process of mechanised verification of their safety and temporal properties.

==> Makefile <==
export TEXINPUTS:=.:formatting:$(TEXINPUTS)

CROSSTEX := crosstex
CROSSTEX_ARGS := --titlecase lower --add-in --short=author --short=conference

BIBTEX   := bibtex

FIGFIGS :=
EPSFIGS := 
PNGFIGS :=
PDFFIGS :=
SVGFIGS := 
GNUPLOTFIGS :=
FIGS    := $(FIGFIGS) $(EPSFIGS) $(PDFFIGS) $(SVGFIGS) $(GNUPLOTFIGS) \
           $(PNGFIGS)

TEX_SOURCES := paper.tex intro.tex related.tex automata.tex defs.tex solidity.tex kick.tex verification.tex parallel.tex conclusion.tex discussion.tex

.SUFFIXES:

all: 
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper
pdf: paper.pdf

zip: Makefile paper.tex intro.tex related.tex automata.tex defs.tex solidity.tex kick.tex verification.tex parallel.tex conclusion.tex discussion.tex   
	zip paper.zip paper.tex intro.tex related.tex automata.tex defs.tex solidity.tex kick.tex verification.tex parallel.tex conclusion.tex discussion.tex Makefile acmart.cls crowd_sol.tex lstcoq.tex mathpartir.sty ref.bib

commit: 
	git commit -m "Update stuff" -a
	git push origin master

pull:
	git pull origin master 

spell: $(TEX_SOURCES)
	detex $^ | spell | env LANG=C sort -u | env LANG=C comm -23 - ok-words

clean:
	rm -f *~ *.log *.bbl *.dvi paper.pdf *.blg *.aux *.ps *.out


==> crowd_sol.tex <==
\begin{figure*}[t]
\centering
%\begin{tabular}{cc}
\begin{minipage}{0.50\linewidth}
{
% ,frame=single, framexleftmargin=20pt,
% framexrightmargin=8cm,framextopmargin=5pt,
% backgroundcolor=\color{light-gray},
\begin{lstlisting}[language=Scilla,numbers=left,mathescape=true, 
basicstyle=\footnotesize\ttfamily]
contract Crowdfunding {
    address public owner;
    uint public goal; 
    uint public max_block;

    // Data structures
    enum State {
        Fundraising,
        ExpiredRefundPending,
        Successful,
        ExpiredRefundComplete
    }
    
    mapping (address => unit) backers;

    // State variables
    State public state = State.Fundraising; 
    uint public totalRaised;
    
    modifier inState(State _state) {
        if (state != _state) throw;
        _
    }

    modifier isowner() {
        if (msg.sender != owner) throw;
        _
    }

    modifier atEndOfLifecycle() {
        if(state != State.ExpiredRefundComplete && 
           state != State.Successful) {
            throw;
        }
    }

    function Crowdfunding(uint _max_block, uint _goal){
        owner = msg.sender;
        goal = _goal;
        max_block = _max_block;
    }
\end{lstlisting}
}
\end{minipage}
%&
\begin{minipage}{0.45\linewidth}
{
\begin{lstlisting}[mathescape=true,language=Scilla,basicstyle=\footnotesize\ttfamily,numbers=left,firstnumber=44]
    function donate() public 
    	inState(State.Fundraising){
        backers[msg.sender] = msg.value;
        totalRaised += msg.value;
		checkIfFundingCompleteOrExpired();
    }

    function checkIfFundingCompleteOrExpired() {
        if (totalRaised > goal) {
            state = State.Successful;
            GetFunds();
        } else if ( block.number > max_block && 
		this.balance > 0 )  {
            state = State.ExpiredRefundPending;
            Claim();
        }
    	else if ( block.number > max_block && 
		this.balance == 0 )  {
            state = State.ExpiredRefundComplete;
    	}
    }

    function GetFunds() public
    	isowner()
    	inState(State.Successful){
        if(!owner.send(this.balance)) {
            throw;
        }
    }

    function Claim() public 
    	inState(State.ExpiredRefundPending){
            if(!msg.sender.send(backers[msg.sender])) {
                throw;
            }
    }

}

\end{lstlisting}
}
\end{minipage}
%\end{tabular}
\caption{\texttt{Crowdfunding} contract in Solidity. We have intentionally
simplified the code so as to exclude events and the call back function.}
\label{fig:kick-sol} 
\end{figure*}


==> parallel.tex <==
\section{Support for High Throughput Applications}
\label{sec:parallel}

==> solidity.tex <==
\section{Translation from Solidity to \scilla}
\label{sec:solidity}

We now briefly outline a relation between smart contracts implemented
Solidity, a high-level smart contract language in Ethereum, and their
translation into \scilla-based representation.

\input{crowd_sol.tex}

Figure~\ref{fig:kick-sol} shows the code of the familiar
\code{Crowdsourcing} contract implemented in Solidity. The following
aspects differ in the two representations.

\paragraph{Constructors.~}

Contracts in \scilla, unlike their counterparts in Solidity do not
have an explicit constructor. In order to initialize a contract, a
user should pass all arguments, corresponding to formal immutable
parameters of the contract. Mutable fields can be instantiated using
expressions that are constants or involve contract's parameters.

\paragraph{Modifiers and throwing exceptions.}

TODO 

\paragraph{Non-tail calls.}

TODO: translate the cycle in the \code{Claim} function


% \is{Key components:}

% \begin{itemize}
% \item CPS
% \item Defunctionalization
% \item Non-continuous control-flow (break/throw)
% \end{itemize}


